RevUp: Revise and Update Information Bottleneck for Event Representation

The existence of external (``side'') semantic knowledge has been shown to result in more expressive computational event models. To enable the use of side information that may be noisy or missing, we propose a semi-supervised information bottleneck-based discrete latent variable model. We reparameterize the model's discrete variables with auxiliary continuous latent variables and a light-weight hierarchical structure. Our model is learned to minimize the mutual information between the observed data and optional side knowledge that is not already captured by the new, auxiliary variables. We theoretically show that our approach generalizes past approaches, and perform an empirical case study of our approach on event modeling. We corroborate our theoretical results with strong empirical experiments, showing that the proposed method outperforms previous proposed approaches on multiple datasets.

==> algorithms/mini_algo.tex <==
\begin{algorithm}[H]
\caption{assignment algorithm}
\begin{algorithmic}
  \State $\bx\sim p_{\mathcal{D}}(\bx)$
  \State $\mathbf{e}=[]$
  \Function{Encoder}{$a$}
  \State $\mathbf{H}\leftarrow \text{RNN}(\bx)$ \Comment{RNN hidden states}
  \State $[\mu_1,\sigma_1]=\text{NN}(\mathbf{H})$ \Comment{Gaussian parameters}
  \State $z_1\sim \mathcal{N}(\mu_1,\sigma_1)$
  \For{$m=1 \text{ to } M$}
    \State $\hat{\lambda}_m \sim \text{Bern}(1/(1+\lambda l_m))$ \Comment{Indicator}
    \State $\gamma_m\leftarrow\text{NN}(z_m)$ \Comment{Gumbel Softmax parameters}
    \State $t_m \sim \hat{\lambda}_m r_{\gamma}(t_m\vert z_m) +(1-\hat{\lambda}_m) p_{\mathcal{D}}(t_m\vert x_m)$ \Comment{Knowledge Sampling} 
    \State $e_m = t_m^T E$ \Comment{Frame embedding}
    \State $\mathbf{e}.\text{append}(e_m)$ \Comment{Collect Embeddings}
    \State $[\mu_{m+1},\sigma_{m+1}] = \text{Attention}(\textbf{H},e_m)$ \Comment{Attention over input data and embedding}
    \State $z_{m+1}\sim \mathcal{N}(\mu_{m+1},\sigma_{m+1})$ \Comment{Sampling new latent}
  \EndFor
  \EndFunction
  \Function{Decoder}{$a$}
  \For{$t=1 \text{ to } T$}
  \State $x_t \sim p(x_t)$
  \EndFor
  \EndFunction
\end{algorithmic}
\end{algorithm}


==> algorithms/new_algo.tex <==
\begin{algorithm}[t]
\caption{Encoder and decoder algorithms}
\begin{algorithmic}
  \State $\bx\sim p_{\mathcal{D}}(\bx)$
  \State $\mathbf{e}=[]$
  \Function{Encoder}{$\bx$}
  \State $\mathbf{H}_{\text{enc}}\leftarrow \text{RNN}(\bx)$ \Comment{Encoder RNN hidden states}
  \State $[\mu_1,\sigma_1]=\text{NN}(\mathbf{H})$ \Comment{Gaussian parameters}
  \State $z_1\sim \mathcal{N}(\mu_1,\sigma_1)$
  \For{$m=1 \text{ to } M$}
    \State $\hat{\lambda}_m \sim \text{Bern}(1/(1+\lambda l_m))$ \Comment{Bernoulli Sampling}
    \State $\gamma_m\leftarrow\text{NN}(z_m)$ \Comment{Gumbel Softmax parameters}
    \State $t_m \sim \hat{\lambda}_m r_{\gamma}(t_m\vert z_m) +(1-\hat{\lambda}_m) p_{\mathcal{D}}(t_m\vert x_m)$ \Comment{Knowledge Sampling} 
    \State $e_m = t_m^T E$ \Comment{Frame embedding}
    \State $\mathbf{e}.\text{append}(e_m)$ \Comment{Collect Embeddings}
    \State $[\mu_{m+1},\sigma_{m+1}] = \text{Attention}(\textbf{H},e_m)$ \Comment{Attention over input data and embedding}
    \State $z_{m+1}\sim \mathcal{N}(\mu_{m+1},\sigma_{m+1})$ \Comment{Sampling new latent}
  \EndFor
  \EndFunction
  \Function{Decoder}{$\mathbf{e}$}
  \For{$t=1 \text{ to } T$}
  \State $h_{\text{dec}}=\text{RNN}(x_{t-1})$
  \State $g=\text{Attention}(h_{\text{dec}},\mathbf{e})$
  \State $x_t \sim p(x_t;g)$
  \EndFor
  \EndFunction
\end{algorithmic}
\end{algorithm}



==> sec_checklist.tex <==
\newpage
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}{}
  \item Did you mention the license of the assets?
    \answerYes{}{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We do not create new datasets.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}{}
\end{enumerate}


\end{enumerate}


==> sec_task_overview.tex <==
\section{Task Overview} 
\label{sec:task-overview}
We consider the task of SE type classification using
the %MASC+Wiki dataset that is publicly available
publicly available MASC+Wiki dataset
\citep{friedrich2016situation}.\footnote{\url{https://github.com/BaokuiWang/context_aware_situation_entity}} %
In this task, an English clause, containing an event-like predicate, is classified into different SE types: states, events, reports, generic sentences,
generalizing sentences, questions, and imperative sentences. %
\cref{fig:model_structure} shows an example of a \textsc{generic}. %
See \Cref{Table:datasets} in the appendix for high-level statistics about the dataset, and \citet{friedrich2016situation} for an in-depth explanation of each of the SE types. %
%This dataset represents documents as a sequence of ``clauses,'' each with their own respective SE type labels. 
%This dataset characterizes the clauses based on their embedded facts they introduce within a text or discourse.
%To further understanding of how different types of situations can be used across domains and writing styles, 
This dataset also segments the documents into their various genres, such as ``email,'' ``fiction,'' and ``technical.''
%  \begin{figure}[t!]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/tsne-mu/1000_adjust.pdf}
%   \caption{Accuracy}
%   \label{fig:OptClsBert}
% \end{figure}
% described below.
% \begin{enumerate}
%     \item EVENT: He punched me.
%     \item STATE: I am here now.
%     \item REPORT: “Thank yocu,” he whispered again.
%     \item GENERIC SENTENCE: He punched me.
%     \item EVENT: He punched me.
% \end{enumerate}


